Sampling for Inference in Probabilistic Models with Fast Bayesian Quadrature

We propose a novel sampling framework for inference in probabilistic models: an active learning approach that converges more quickly (in wall-clock time) than Markov chain Monte Carlo (MCMC) benchmarks. The central challenge in probabilistic inference is numerical integration, to average over ensembles of models or unknown (hyper-)parameters (for example to compute the marginal likelihood or a partition function). MCMC has provided approaches to numerical integration that deliver state-of-the-art inference, but can suffer from sample inefficiency and poor convergence diagnostics. Bayesian quadrature techniques offer a model-based solution to such problems, but their uptake has been hindered by prohibitive computation costs. We introduce a warped model for probabilistic integrands (likelihoods) that are known to be non-negative, permitting a cheap active learning scheme to optimally select sample locations. Our algorithm is demonstrated to offer faster convergence (in seconds) relative to simple Monte Carlo and annealed importance sampling on both synthetic and real-world examples.

==> finalplots/bqfunconly.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{5}{5}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA True function}%
\psfrag{001}[cl][cl]{\matlabtextA \textsc{gp}\xspace posterior mean}%
\psfrag{002}[cl][cl]{\matlabtextA 95\% confidence interval}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{003}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{004}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/bqfunconlynosamples.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA True Function}%
\psfrag{001}[cl][cl]{\matlabtextA GP Posterior Mean}%
\psfrag{002}[cl][cl]{\matlabtextA 95% Confidence Interval}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{20}{20}\selectfont\strut}%
\psfrag{003}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{004}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/bqfuncppriornosamples.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA True Function}%
\psfrag{001}[cl][cl]{\matlabtextA GP Posterior Mean}%
\psfrag{002}[cl][cl]{\matlabtextA 95% Confidence Interval}%
\psfrag{003}[cl][cl]{\matlabtextA Prior Mass}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{20}{20}\selectfont\strut}%
\psfrag{004}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{005}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/bqfunpprior.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA Sample Locations}%
\psfrag{001}[cl][cl]{\matlabtextA True Function}%
\psfrag{002}[cl][cl]{\matlabtextA GP Posterior Mean}%
\psfrag{003}[cl][cl]{\matlabtextA 95% Confidence Interval}%
\psfrag{004}[cl][cl]{\matlabtextA Prior Mass}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{20}{20}\selectfont\strut}%
\psfrag{005}[bc][bc]{\matlabtextB $\elll(x)$}%
\psfrag{006}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/gmmerrormoment.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA SMC 1 Standard Deviation}%
\psfrag{009}[cl][cl]{\matlabtextA SMC}%
\psfrag{010}[cl][cl]{\matlabtextA \moment_sqrt 1 Standard Deviation}%
\psfrag{011}[cl][cl]{\matlabtextA \moment_sqrt}%
\psfrag{012}[bc][bc]{\matlabtextA Fractional error vs ground truth}%
\psfrag{013}[tc][tc]{\matlabtextA Time in seconds}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $50$}%
\psfrag{002}[ct][ct]{\matlabtextA $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextA $10^{-4}$}%
\psfrag{004}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{005}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{006}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{007}[rc][rc]{\matlabtextA $10^{0}$}%
%
%% </ytick>

==> finalplots/gmmlikelihoodmoment.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA SMC}%
\psfrag{013}[cl][cl]{\matlabtextA \moment_sqrt}%
\psfrag{014}[bc][bc]{\matlabtextA Average likelihood of ground truth}%
\psfrag{015}[tc][tc]{\matlabtextA Time in seconds}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $50$}%
\psfrag{002}[ct][ct]{\matlabtextA $100$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{003}[bc][bc]{\matlabtextA $\times10^{6}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextA $0$}%
\psfrag{005}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{006}[rc][rc]{\matlabtextA $1$}%
\psfrag{007}[rc][rc]{\matlabtextA $1.5$}%
\psfrag{008}[rc][rc]{\matlabtextA $2$}%
\psfrag{009}[rc][rc]{\matlabtextA $2.5$}%
\psfrag{010}[rc][rc]{\matlabtextA $3$}%
\psfrag{011}[rc][rc]{\matlabtextA $3.5$}%
%
%% </ytick>

==> finalplots/heatmap2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA 95\% Confidence Interval \linearsqrt}%
\psfrag{001}[cl][cl]{\matlabtextA Posterior Mean \linearsqrt}%
\psfrag{002}[cl][cl]{\matlabtextA Ground Truth}%
\psfrag{003}[cl][cl]{\matlabtextA 95\% Confidence Interval \momentsqrt}%
\psfrag{004}[cl][cl]{\matlabtextA Posterior Mean \momentsqrt}%
\psfrag{005}[cl][cl]{\matlabtextA Simulated \chi^2 process}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{20}{20}\selectfont\strut}%
\psfrag{006}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{007}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/heatmap3.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA 95\% Confidence Interval \linearsqrt}%
\psfrag{001}[cl][cl]{\matlabtextA Posterior Mean \linearsqrt}%
\psfrag{002}[cl][cl]{\matlabtextA Ground Truth}%
\psfrag{003}[cl][cl]{\matlabtextA 95\% Confidence Interval \momentsqrt}%
\psfrag{004}[cl][cl]{\matlabtextA Posterior Mean \momentsqrt}%
\psfrag{005}[cl][cl]{\matlabtextA Simulated \chi^2 process}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{20}{20}\selectfont\strut}%
\psfrag{006}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{007}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/heatmap4.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA 95\% Confidence Interval \linearsqrt}%
\psfrag{001}[cl][cl]{\matlabtextA Posterior Mean \linearsqrt}%
\psfrag{002}[cl][cl]{\matlabtextA Ground Truth}%
\psfrag{003}[cl][cl]{\matlabtextA 95\% Confidence Interval \momentsqrt}%
\psfrag{004}[cl][cl]{\matlabtextA Posterior Mean \momentsqrt}%
\psfrag{005}[cl][cl]{\matlabtextA Simulated \chi^2 process}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{20}{20}\selectfont\strut}%
\psfrag{006}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{007}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/heatmap5.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA 95\% Confidence Interval \linear_sqrt}%
\psfrag{001}[cl][cl]{\matlabtextA Posterior Mean \linear_sqrt}%
\psfrag{002}[cl][cl]{\matlabtextA Ground Truth}%
\psfrag{003}[cl][cl]{\matlabtextA 95\% Confidence Interval \moment_sqrt}%
\psfrag{004}[cl][cl]{\matlabtextA Posterior Mean \moment_sqrt}%
\psfrag{005}[cl][cl]{\matlabtextA Simulated \chi^2 process}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{20}{20}\selectfont\strut}%
\psfrag{006}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{007}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/heatmap6.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA 95\% Confidence Interval \linear_sqrt}%
\psfrag{001}[cl][cl]{\matlabtextA Posterior Mean \linear_sqrt}%
\psfrag{002}[cl][cl]{\matlabtextA Ground Truth}%
\psfrag{003}[cl][cl]{\matlabtextA 95\% Confidence Interval \moment_sqrt}%
\psfrag{004}[cl][cl]{\matlabtextA Posterior Mean \moment_sqrt}%
\psfrag{005}[cl][cl]{\matlabtextA Simulated \chi^2 process}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{20}{20}\selectfont\strut}%
\psfrag{006}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{007}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/linearbqactivesamples.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{4.8}{8}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA Optimal Next Sample}%
\psfrag{001}[cl][cl]{\matlabtextA True Function}%
\psfrag{002}[cl][cl]{\matlabtextA \linearsqrt Posterior Mean}%
\psfrag{003}[cl][cl]{\matlabtextA 95\% Confidence Interval}%
\psfrag{004}[cl][cl]{\matlabtextA Prior Mass}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{005}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{006}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/linsqrtbqfunconlynosamples.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA True Function}%
\psfrag{001}[cl][cl]{\matlabtextA \linear_sqrt Posterior Mean}%
\psfrag{002}[cl][cl]{\matlabtextA 95% Confidence Interval}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{20}{20}\selectfont\strut}%
\psfrag{003}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{004}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/linsqrtbqfuncppriornosamples.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA True Function}%
\psfrag{001}[cl][cl]{\matlabtextA \linear_sqrt Posterior Mean}%
\psfrag{002}[cl][cl]{\matlabtextA 95% Confidence Interval}%
\psfrag{003}[cl][cl]{\matlabtextA Prior Mass}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{20}{20}\selectfont\strut}%
\psfrag{004}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{005}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/linsqrtbqoptnextsamp.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA Optimal Next Sample}%
\psfrag{001}[cl][cl]{\matlabtextA True Function}%
\psfrag{002}[cl][cl]{\matlabtextA \linear_sqrt Posterior Mean}%
\psfrag{003}[cl][cl]{\matlabtextA 95% Confidence Interval}%
\psfrag{004}[cl][cl]{\matlabtextA Prior Mass}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{20}{20}\selectfont\strut}%
\psfrag{005}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{006}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/momentbqactivesamples.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{5}{5}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA True Function}%
\psfrag{001}[cl][cl]{\matlabtextA GP Posterior Mean}%
\psfrag{002}[cl][cl]{\matlabtextA 95% Confidence Interval}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{003}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{004}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/momentsqrtbqfunconly.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}}%
\psfrag{000}[cl][cl]{\matlabtextA True Function}%
\psfrag{001}[cl][cl]{\matlabtextA \momentsqrt Posterior Mean}%
\psfrag{002}[cl][cl]{\matlabtextA 95\% Confidence Interval}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}}%
\psfrag{003}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{004}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/momentsqrtbqfunconlynosamples.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{5}{5}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA True Function}%
\psfrag{001}[cl][cl]{\matlabtextA \momentsqrt Posterior Mean}%
\psfrag{002}[cl][cl]{\matlabtextA 95\% Confidence Interval}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{003}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{004}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/momentsqrtbqfuncppriornosamples.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA True Function}%
\psfrag{001}[cl][cl]{\matlabtextA \moment_sqrt Posterior Mean}%
\psfrag{002}[cl][cl]{\matlabtextA 95% Confidence Interval}%
\psfrag{003}[cl][cl]{\matlabtextA Prior Mass}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{20}{20}\selectfont\strut}%
\psfrag{004}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{005}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/momentsqrtbqoptnextsamp.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA Optimal Next Sample}%
\psfrag{001}[cl][cl]{\matlabtextA True Function}%
\psfrag{002}[cl][cl]{\matlabtextA \moment_sqrt Posterior Mean}%
\psfrag{003}[cl][cl]{\matlabtextA 95% Confidence Interval}%
\psfrag{004}[cl][cl]{\matlabtextA Prior Mass}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{20}{20}\selectfont\strut}%
\psfrag{005}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{006}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>

==> finalplots/momentsqrtfunconly.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{5}{5}\selectfont\strut}%
\psfrag{000}[cl][cl]{\matlabtextA True function}%
\psfrag{001}[cl][cl]{\matlabtextA \momentsqrt posterior mean}%
\psfrag{002}[cl][cl]{\matlabtextA 95\% confidence interval}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{003}[bc][bc]{\matlabtextB $\ell(x)$}%
\psfrag{004}[tc][tc]{\matlabtextB $\mathcal{X}$}%
%
%% </text>


==> finalplots/nipsclassresults.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{6}{6}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA \textsc{bmc}}%
\psfrag{017}[cl][cl]{\matlabtextA \textsc{ais}}%
\psfrag{018}[cl][cl]{\matlabtextA \textsc{smc}}%
\psfrag{019}[cl][cl]{\matlabtextA \momentsqrt}%
\psfrag{020}[cl][cl]{\matlabtextA \linearsqrt}%
\psfrag{021}[cl][cl]{\matlabtextA Ground truth}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{022}[bc][bc]{\matlabtextB $\log Z$}%
\psfrag{023}[tc][tc]{\matlabtextB Time in seconds}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{6}{6}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $200$}%
\psfrag{001}[ct][ct]{\matlabtextC $400$}%
\psfrag{002}[ct][ct]{\matlabtextC $600$}%
\psfrag{003}[ct][ct]{\matlabtextC $800$}%
\psfrag{004}[ct][ct]{\matlabtextC $1000$}%
\psfrag{005}[ct][ct]{\matlabtextC $1200$}%
\psfrag{006}[ct][ct]{\matlabtextC $1400$}%
\psfrag{007}[ct][ct]{\matlabtextC $1600$}%
\psfrag{008}[ct][ct]{\matlabtextC $1800$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextC $-300$}%
\psfrag{010}[rc][rc]{\matlabtextC $-290$}%
\psfrag{011}[rc][rc]{\matlabtextC $-280$}%
\psfrag{012}[rc][rc]{\matlabtextC $-270$}%
\psfrag{013}[rc][rc]{\matlabtextC $-260$}%
\psfrag{014}[rc][rc]{\matlabtextC $-250$}%
\psfrag{015}[rc][rc]{\matlabtextC $-240$}%
%
%% </ytick>


==> finalplots/syntheticresults.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{6}{6}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA BMC}%
\psfrag{011}[cl][cl]{\matlabtextA AIS}%
\psfrag{012}[cl][cl]{\matlabtextA SMC}%
\psfrag{013}[cl][cl]{\matlabtextA \momentsqrt}%
\psfrag{014}[cl][cl]{\matlabtextA \linearsqrt}%
\psfrag{015}[cl][cl]{\matlabtextA Ground truth}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{6}{6}\selectfont\strut}%
\psfrag{016}[bc][bc]{\matlabtextB $\log Z$}%
\psfrag{017}[tc][tc]{\matlabtextB Time in seconds}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{6}{6}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $100$}%
\psfrag{002}[ct][ct]{\matlabtextC $200$}%
\psfrag{003}[ct][ct]{\matlabtextC $300$}%
\psfrag{004}[ct][ct]{\matlabtextC $400$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $-160$}%
\psfrag{006}[rc][rc]{\matlabtextC $-158$}%
\psfrag{007}[rc][rc]{\matlabtextC $-156$}%
\psfrag{008}[rc][rc]{\matlabtextC $-154$}%
\psfrag{009}[rc][rc]{\matlabtextC $-152$}%
%
%% </ytick>


==> finalplots/syntheticresults2.oldtex.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{6}{6}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA \textsc{bmc}}%
\psfrag{015}[cl][cl]{\matlabtextA \textsc{ais}}%
\psfrag{016}[cl][cl]{\matlabtextA \textsc{smc}}%
\psfrag{017}[cl][cl]{\matlabtextA \momentsqrt}%
\psfrag{018}[cl][cl]{\matlabtextA \linearsqrt}%
\psfrag{019}[cl][cl]{\matlabtextA Ground truth}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextB logZ}%
\psfrag{021}[tc][tc]{\matlabtextB Time in seconds}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{6}{6}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $50$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
\psfrag{003}[ct][ct]{\matlabtextC $150$}%
\psfrag{004}[ct][ct]{\matlabtextC $200$}%
\psfrag{005}[ct][ct]{\matlabtextC $250$}%
\psfrag{006}[ct][ct]{\matlabtextC $300$}%
\psfrag{007}[ct][ct]{\matlabtextC $350$}%
\psfrag{008}[ct][ct]{\matlabtextC $400$}%
\psfrag{009}[ct][ct]{\matlabtextC $450$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextC $-160$}%
\psfrag{011}[rc][rc]{\matlabtextC $-155$}%
\psfrag{012}[rc][rc]{\matlabtextC $-150$}%
\psfrag{013}[rc][rc]{\matlabtextC $-145$}%
%
%% </ytick>


==> finalplots/yachtresults.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{7}\selectfont\strut}%
\psfrag{015}[cl][cl]{\matlabtextA \textsc{bmc}}%
\psfrag{016}[cl][cl]{\matlabtextA \textsc{ais}}%
\psfrag{017}[cl][cl]{\matlabtextA \textsc{smc}}%
\psfrag{018}[cl][cl]{\matlabtextA \momentsqrt}%
\psfrag{019}[cl][cl]{\matlabtextA \linearsqrt}%
\psfrag{020}[cl][cl]{\matlabtextA Ground truth}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{7}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextA logZ}%
\psfrag{022}[tc][tc]{\matlabtextA Time in seconds}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{7}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $200$}%
\psfrag{002}[ct][ct]{\matlabtextA $400$}%
\psfrag{003}[ct][ct]{\matlabtextA $600$}%
\psfrag{004}[ct][ct]{\matlabtextA $800$}%
\psfrag{005}[ct][ct]{\matlabtextA $1000$}%
\psfrag{006}[ct][ct]{\matlabtextA $1200$}%
\psfrag{007}[ct][ct]{\matlabtextA $1400$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{008}[bc][bc]{\matlabtextA $\times10^{4}$}%
%
%% </yscale>
%
%% <ytick>
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{7}{7}\selectfont\strut}%
\psfrag{009}[rc][rc]{\matlabtextA $-1.5$}%
\psfrag{010}[rc][rc]{\matlabtextA $-1$}%
\psfrag{011}[rc][rc]{\matlabtextA $-0.5$}%
\psfrag{012}[rc][rc]{\matlabtextA $0$}%
\psfrag{013}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{014}[rc][rc]{\matlabtextA $1$}%
%
%% </ytick>
